On the Role of Visual Cues in Audiovisual Speech Enhancement

We present an introspection of an audiovisual speech enhancement model. In particular, we focus on interpreting how a neural audiovisual speech enhancement model uses visual cues to improve the quality of the target speech signal. We show that visual cues provide not only high-level information about speech activity, i.e., speech/silence, but also fine-grained visual information about the place of articulation. One byproduct of this finding is that the learned visual embeddings can be used as features for other visual speech applications. We demonstrate the effectiveness of the learned visual embeddings for classifying visemes (the visual analogy to phonemes). Our results provide insight into important aspects of audiovisual speech enhancement and demonstrate how such models can be used for self-supervision tasks for visual speech applications.

==> related.tex <==
% !TEX root = ../main.tex
Past work has shown that the introduction of visual cues can improve the robustness of various speech processing applications. These include automatic speech recognition (ASR), speaker recognition and diarization, speech enhancement, and emotion recognition~\cite{abdelaziz2017comparing,afouras2018deep,abdelaziz2017improving,chung2019said}. This section covers recent relevant works on audiovisual speech enhancement, audiovisual source separation, and speech driven multi-modal self-supervised learning.

Gabbay et al.~introduced an audiovisual speech enhancement model based on an encoder-decoder architecture~\cite{gabbay2017visual}. The model they introduced takes in the log Mel-scale spectrogram representation of the speech segment and the corresponding gray-scale video frames containing the lips of the target speaker to enhance the speech segment. While promising, the models were all speaker-dependent (i.e.,\ the same target speakers were used during training and testing phases), which limits their generalizability.

Ephrat et al.~introduced a speaker-independent approach for audiovisual speech enhancement~\cite{ephrat2018looking}.  Their models take in, as input, a complex-valued spectrogram of a three-second segment of speech and the corresponding video frames cropped to contain only the face, and outputs complex masks, which are used to reconstruct an enhanced speech signal.   Concurrently, Afouras et al.~introduced an audiovisual speech enhancement approach to model both the magnitude and the phase components of the short-time Fourier transform (STFT) representation of the input signal~\cite{afouras2018conversation}.  In a follow-up study, they extended their original approach to make the enhancement model robust to partial occlusions by conditioning it on both visual cues and speaker representations~\cite{afouras2019my}.

Previous research looked at using correlation between acoustic and visual modalities as a self-supervisory training signal~\cite{chung2016out,owens2018audio,zhao2018sound,zhao2019sound,gan2020music}.   Cheng and Zisserman~\cite{chung2016out} trained a model to determine whether the acoustic and visual modalities of a speaker are temporally aligned or not. They created training examples by randomly introducing shifts in one of the modalities. The authors showed that the learned visual representations can be used as features for lip reading applications.  Owens and Efros~\cite{owens2018audio} trained a more general model to predict whether the visual and acoustics streams of a scene are temporally aligned or not, and then used the learned representations for three tasks: source localization, audiovisual action recognition, and audio source separation. 
To the best of our knowledge, our work in this paper is the first to investigate audiovisual speech enhancement as a self-supervisory signal for learning strong visual features.

In contrast to previous research, our work focuses on interpreting how audiovisual enhancers use visual cues to enhance the target signal. The novelty of our work is two-fold. Firstly, we show that the performance of audiovisual speech enhancers varies depending on what is being said, and we show that performance gains vary as a function of the place of articulation. 
Secondly, we demonstrate the effectiveness of the audiovisual speech enhancement task as a self-supervised way of learning useful visual embeddings that encode information about the place of articulation. In the self-supervised paradigm, we learn meaningful representations by training a model to solve a task with labels obtained from the data itself as opposed to labels obtained from manual annotation~\cite{zhang2016colorful}.

% Secondly, we show that audiovisual speech enhancement can be used for self-supervised learning of visual embeddings that encode the place of articulation. We demonstrate the effectiveness of these visual embeddings by training a viseme classifier using them.

